Behavioural Models for Group Communications

Group communication is becoming a more and more popular infrastructure for efficient distributed applications. It consists in representing locally a group of remote objects as a single object accessed in a single step; communications are then broadcasted to all members. This paper provides models for automatic verification of group-based applications, typically for detecting deadlocks or checking message ordering. We show how to encode group communication, together with different forms of synchronisation for group results. The proposed models are parametric such that, for example, different group sizes or group members could be experimented with the minimum modification of the original model.

==> eptcsdata.tex <==
\providecommand{\firstpage}{42}
\providecommand{\publicationstatus}{C\'amara, Canal, and Sala\"un (Eds.) \\
Component and Service Interoperability (WCSI10)\\
EPTCS 37, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.37.4}{10.4204/EPTCS.37.4}}
\pdfoutput=1

